The first measurements of carbon isotopic ratios in post-RGB stars: SZ Mon and DF Cyg. E-iSpec: A spectral analysis tool to derive elemental abundances and isotopic ratios for evolved stars

Dusty post-red giant branch (post-RGB) stars are low- and intermediate-mass stars where the RGB evolution was prematurely terminated by a poorly understood binary interaction. These binary stars are considered to be low-luminosity analogues of post-asymptotic giant branch (post-AGB) binary stars. In this study, we investigated the chemical composition of two dusty post-RGB binary stars, SZ Mon and DF Cyg, using multi-wavelength spectroscopic data from HERMES/Mercator (optical) and the APOGEE survey (near-infrared). Owing to challenges posed by existing spectral analysis tools for the study of evolved stars with complex atmospheres, we developed E-iSpec: a dedicated spectral analysis tool for evolved stars, to consistently determine atmospheric parameters, elemental abundances, and carbon isotopic ratios. Our abundance analysis revealed that observed depletion patterns and estimated depletion efficiencies resemble those found in post-AGB binary stars. However, the onset of chemical depletion in post-RGB targets occurs at higher condensation temperatures ($T_{\rm turn-off, post-RGB}\approx1400$ K), than in most post-AGB stars ($T_{\rm turn-off, post-AGB}\approx1100$ K). Additionally, our study resulted in the first estimates of carbon isotopic ratios for post-RGB stars ($^{12}$C/$^{13}$C$_{\rm SZ Mon}=8\pm4$, $^{12}$C/$^{13}$C$_{\rm DF Cyg}=12\pm3$). We found that the observationally derived CNO abundances and the carbon isotopic ratios of our post-RGB binary targets are in good agreement with theoretical predictions from the ATON single star evolutionary models involving first dredge-up and moderately-deep extra mixing. This agreement emphasises that in post-RGB binary targets, the observed CNO abundances reflect the chemical composition expected from single star nucleosynthesis (i.e., convective and non-convective mixing processes) occurring during the RGB phase before it is terminated.

==> Tables/TablePhoMagFull.tex <==
\begin{landscape}
\begin{table}
    \centering
    \caption{Photometric properties of SZ Mon and DF Cyg.}\label{tab:phomagfull}
    \begin{tabular}{|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
    \hline
        Filter & JOHNSON.U & JOHNSON.B & JOHNSON.B & JOHNSON.B & JOHNSON.B & JOHNSON.B & JOHNSON.V & JOHNSON.V & JOHNSON.V & JOHNSON.V & JOHNSON.V & JOHNSON.V & SDSS.RP & COUSINS.R & JOHNSON.R & COUSINS.I & COUSINS.I & 2MASS.J & 2MASS.H & 2MASS.KS & WISE.W1 & WISE.W2 & MSX.A & AKARI.S9W & WISE.W3 & MSX.C & MSX.D & AKARI.L18W & MSX.E & WISE.W4 \\
        Unit & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & Jy & Jy & mag & Jy & Jy & Jy & Jy & mag \\ \hline
        Wavelength ($\mu$m) & 0.36373 & 0.443354 & 0.443354 & 0.443354 & 0.443354 & 0.443354 & 0.549292 & 0.549292 & 0.549292 & 0.549292 & 0.549292 & 0.549292 & 0.62472 & 0.647294 & 0.689902 & 0.787479 & 0.787479 & 1.23931 & 1.64949 & 2.16386 & 3.34597 & 4.59522 & 8.48032 & 8.85203 & 11.5485 & 12.1516 & 14.6783 & 18.9186 & 21.5008 & 22.0789 \\ \hline
        SZ Mon & 11.097$\pm$0.10728 & 11.328$\pm$0.078 & 10.537$\pm$0.10728 & 10.642$\pm$0.151 & 11.59$\pm$0.08 & 11.321$\pm$NG & 10.29$\pm$NG & 10.38$\pm$0.046 & 9.977$\pm$0.377 & 9.79$\pm$0.03 & 10.152$\pm$0.346 & 10.39$\pm$NG & 10.017$\pm$0.314 & 10.4$\pm$NG & 9.81$\pm$NG & 9.109$\pm$NG & 8.973$\pm$0.354 & 8.675$\pm$0.029 & 8.057$\pm$0.067 & 7.507$\pm$0.027 & 6.621$\pm$0.039 & 5.655$\pm$0.026 & 1.682$\pm$0.068962 & 2.615$\pm$0.0429 & 3.575$\pm$0.014 & 1.844$\pm$0.11064 & 1.212$\pm$0.08484 & 1.585$\pm$0.0404 & 1.382$\pm$0.111942 & 2.413$\pm$0.019 \\
        DF Cyg & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & mag & Jy & Jy & mag & Jy & Jy & Jy & Jy & mag \\ \hline
    \end{tabular}
\end{table}
\end{landscape}
